Generalizing the Network Scale-Up Method: A New Estimator for the Size of Hidden Populations

The network scale-up method enables researchers to estimate the size of hidden populations, such as drug injectors and sex workers, using sampled social network data. The basic scale-up estimator offers advantages over other size estimation techniques, but it depends on problematic modeling assumptions. We propose a new generalized scale-up estimator that can be used in settings with non-random social mixing and imperfect awareness about membership in the hidden population. Further, the new estimator can be used when data are collected via complex sample designs and from incomplete sampling frames. However, the generalized scale-up estimator also requires data from two samples: one from the frame population and one from the hidden population. In some situations these data from the hidden population can be collected by adding a small number of questions to already planned studies. For other situations, we develop interpretable adjustment factors that can be applied to the basic scale-up estimator. We conclude with practical recommendations for the design and analysis of future studies.

==> tables/compoundratio-nsum-bias-cvs-qoi.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-0 package
% Fri Jan 22 05:19:19 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrl}
  \hline
qoi & $\widehat{\text{cv}}$ & source \\ 
  \hline
sex workers & 0.11 & Rwanda \\ 
  msm & 0.50 & Rwanda \\ 
  idu & 0.44 & Rwanda \\ 
  clients of sex workers & 0.12 & Rwanda \\ 
  heavy drug users & 0.10 & Curitiba \\ 
  sex workers & 0.14 & Curitiba \\ 
  msm & 0.10 & Curitiba \\ 
  hiv positive & 0.10 & US \\ 
  homeless & 0.12 & US \\ 
  women raped & 0.17 & US \\ 
   \hline
\end{tabular}
\caption{TODO} 
\label{tab:nsumqoicvs}
\end{table}


==> tables/estimator-sensitivity.tex <==

\begin{table}[h]
\centering
\scalebox{0.7}{
\begin{tabular}{>{\compress}p{3cm} >{\compress}p{9cm} >{\compress}p{4cm}}
\toprule
Quantity & Conditions required & Effective estimand \par for sensitivity analysis\\
\midrule
%%%%%%%% components
reported\par
connections to $H$\par
($\widehat{y}_{F,H}$) &
%\begin{enumerate}[(i)]
\begin{enumerate}
\item probability sample from $F$
\item no false positive reports about connections to $H$ \par ($\eta_F = 1$)
\end{enumerate} 
&
$ \widehat{y}_{F,H} \leadsto \eta_F N_H $
%Result~\ref{res:estimator-yft}
\\
\midrule
average personal network size of $F$\par
($\widehat{\bar{d}}_{F,F}$) &
%\begin{enumerate}[(i)]
\begin{enumerate}
\item probability sample from $F$
\item accurate groups of known size total \par($\widehat{N}_\mathcal{A} = c_1 N_\mathcal{A}$)
\item probe alter condition \par($\bar{d}_{\mathcal{A},F}=c_2 \bar{d}_{F,F}$)
\item accurate reporting condition \par($y_{F,\mathcal{A}} = c_3 d_{F,\mathcal{A}}$)
\end{enumerate} 
&
$\widehat{\bar{d}}_{F,F} \leadsto \frac{c_2 c_3}{c_1} \bar{d}_{F,F}
%Result~\ref{res:kpestimator-dff}
\\
\midrule
average\par 
visibility of $H$\par
($\widehat{\bar{v}}_{H,F}$) &
%\begin{enumerate}[(i)]
\begin{enumerate}
\item relative probability sample from $H$
\item accurate groups of known size total \par
    ($\widehat{N}_{\mathcal{A}_H} = c_1 N_{\mathcal{A}_H}$)
\item probe alter condition \par
    ($\frac{v_{\mathcal{A}\cap F,H}}{N_{\mathcal{A}\cap F}} = 
    c_2 \frac{v_{H,F}}{N_F}$)
\item accurate aggregate reports about visibility \par
    ($\tilde{v}_{H, \mathcal{A}_H \cap F} = c_3 v_{H, \mathcal{A}_H \cap F}$)
\end{enumerate} 
&
$\widehat{\bar{v}}_{H,F} \leadsto \frac{c_2 c_3}{c_1} \bar{v}_{H,F}$
%Result~\ref{res:goc-v-estimator}
\\
\midrule
\midrule
%%%%%%%% estimators
generalized\par 
scale-up\par
($\widehat{N}_{H} = \frac{\widehat{y}_{F,H}}{\widehat{\bar{v}}_{H,F}}$)&
%\begin{enumerate}[(i)]
\begin{enumerate}
    \item conditions needed for $\widehat{y}_{F,H}$ \par
          ($\widehat{y}_{F,H} = \tau_F y_{F,H}$)
    \item conditions needed for $\widehat{\bar{v}}_{H,F}$ \par
          ($\widehat{\bar{v}}_{F,H} = c_1 \bar{v}_{F,H}$)
\end{enumerate} 
&
$\widehat{N}_H \leadsto \frac{\tau_F}{c_1} N_H$
%Result~\ref{res:goc-gnsum-new}
\\
\midrule
modified\par
basic scale-up\par
($\widehat{N}_{H} = \frac{\widehat{y}_{F,H}}{\widehat{\bar{d}}_{F,F}}$) &
%\begin{enumerate}[(i)]
\begin{enumerate}
    \item conditions needed for $\widehat{y}_{F,H}$ \par
          ($\widehat{y}_{F,H} = \tau_F y_{F,H}$)
    \item condition needed for $\widehat{\bar{d}}_{F,F}$ \par
          ($\widehat{\bar{d}}_{F,F} = c_1 \bar{d}_{F,F}$)
    \item personal networks of $H$ are the same average size as personal networks of $F$ \par ($\delta_F \neq 1$)
    \item no false negative reports about connections to $H$ \par ($\tau_F \neq 1$)
\end{enumerate} 
&
$\widehat{N}_H \leadsto \frac{\tau_F}{c_1 \delta_F \tau_F} N_H$
%Sections~\ref{sec:framework}-\ref{sec:relationshiptoscaleup}
\\
\bottomrule
\end{tabular}
}
\caption{Summary of the sensitivity of the basic and generalized network
    scale-up estimators, and their components, to the conditions needed to
    produce estimates that are consistent and essentially unbiased. This table
    uses the version of the basic scale-up estimator we recommend in
    Section~\ref{sec:recommendation-only-sf}. For the basic scale-up estimator,
    if the adjustment factors $\tau_F$ and $\delta_F$ exactly cancel, so that
    $\frac{1}{\delta_F}=\tau_F$, then they do not both need to be equal to 1. }
\label{tab:overall-sensitivity}
\end{table}	



==> tables/gnsum-cv-table.tex <==
% latex table generated in R 3.0.1 by xtable 1.7-1 package
% Wed Oct  2 23:43:19 2013
\begin{table}[ht]
\centering
\begin{tabular}{rllr}
  \hline
 & source & qoi & cv \\ 
  \hline
1 & Rwanda & sex.workers & 0.05 \\ 
  2 & Rwanda & msm & 0.20 \\ 
  3 & Rwanda & idu & 0.24 \\ 
  4 & Rwanda & clients & 0.08 \\ 
  5 & Curitiba & heavy.drug.user & 0.06 \\ 
  6 & Curitiba & sex.worker & 0.13 \\ 
  7 & Curitiba & man.sex.men & 0.09 \\ 
  8 & US & hiv & 0.10 \\ 
  9 & US & homeless & 0.12 \\ 
  10 & US & raped & 0.17 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/maintext-sensitivity.tex <==
% see
% http://tex.stackexchange.com/questions/6445/preventing-itemize-environment-to-insert-initial-vertical-space
% for helpful info on inserting itemized lists in tables

\begin{table}
\centering
\begin{tabular}{l >{\compress}p{4cm} p{3.5cm}}
\toprule
Estimator & Imperfect assumptions & Effective estimand\\
\midrule

%%%%%%%% basic scale-up
$\widehat{N}_{H}$ (basic scale-up) &
\begin{enumerate}[(i)]
\item $\widehat{N}_\mathcal{A} = c_1 ~N_\mathcal{A}$
\item $\bar{d}_{\mathcal{A}, F} = c_2 ~\bar{d}_{F,F}$
\item $y_{F, \mathcal{A}} = c_3 ~ d_{F, \mathcal{A}}$
\end{enumerate} 
&
$\frac{c_2~c_3}{c_1} ~\bar{d}_{F,F}$\\
\midrule
%%%%%%%% generalized scale-up
$\widehat{N}_{H}$ (generalized scale-up) &
\begin{enumerate}[(i)]
\item $\widehat{N}_\mathcal{A} = c_1 ~N_\mathcal{A}$
\item $\bar{d}_{\mathcal{A}, F} = c_2 ~\bar{d}_{U,F}$
\item $y_{F, \mathcal{A}} = c_3 ~ d_{F, \mathcal{A}}$
\end{enumerate} 
&
$\frac{c_2~c_3}{c_1} ~\bar{d}_{U,F}$\\
\bottomrule

\end{tabular}
\caption{TODO.}
\label{tab:size-estimate-sensitivity}
\end{table}	

